EBS-EKF: Accurate and High Frequency Event-based Star Tracking

Event-based sensors (EBS) are a promising new technology for star tracking due to their low latency and power efficiency, but prior work has thus far been evaluated exclusively in simulation with simplified signal models. We propose a novel algorithm for event-based star tracking, grounded in an analysis of the EBS circuit and an extended Kalman filter (EKF). We quantitatively evaluate our method using real night sky data, comparing its results with those from a space-ready active-pixel sensor (APS) star tracker. We demonstrate that our method is an order-of-magnitude more accurate than existing methods due to improved signal modeling and state estimation, while providing more frequent updates and greater motion tolerance than conventional APS trackers. We provide all code and the first dataset of events synchronized with APS solutions.

==> graphics/algorithms/update_algorithm.tex <==





==> graphics/tables/dataset_algorithm_table_v1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\small
\begin{tabular}{@{}lllll|lll@{}}
\toprule
\multicolumn{1}{c|}{}                                                                                                    &                                                                               & \multicolumn{3}{c|}{\textbf{Algorithmic Details}}                                                                                                                                                                                                                                                                                            & \multicolumn{3}{c}{\textbf{Evaluation on Night Sky Data}}                                                                                                                                                                                                                                                            \\ \cmidrule(l){2-8} 
\multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}DVS Star Tracking\\  Algorithm\end{tabular}}}}   & \cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}l@{}}State \\ Est.\end{tabular} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Absolute Orientation\\ Updates\end{tabular}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Centroiding \\ Method\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Original\\  Evaluation\end{tabular}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Max Slew\\  Rate\end{tabular}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Update\\  Rate\end{tabular}} & \multicolumn{1}{c}{\cellcolor[HTML]{C0C0C0}\begin{tabular}[c]{@{}c@{}}Tracking \\ Accuracy\end{tabular}} \\ \midrule
\cellcolor[HTML]{656565}{\color[HTML]{EFEFEF} \begin{tabular}[c]{@{}l@{}}Iterative Closest \\ Points (ICP)\end{tabular}} & 2D                                                                            & \begin{tabular}[c]{@{}l@{}}Required\\ often\end{tabular}                                                           & Center of All Events                                                                                      & LCD Screen                                                                                                  & \textless 5 deg/s                                                                                    & \begin{tabular}[c]{@{}l@{}}40ms \\ / 25Hz\end{tabular}                                             & $\sim$3,000 arcsecs                                                                                      \\
\cellcolor[HTML]{656565}{\color[HTML]{EFEFEF} \begin{tabular}[c]{@{}l@{}}Hough Transform \\ (HT)\end{tabular}}           & 2D                                                                            & \begin{tabular}[c]{@{}l@{}}Required \\ intermittently\end{tabular}                                                 & Center of Positive Events                                                                                 & LCD Screen                                                                                                  & \textless 5 deg/s                                                                                    & \begin{tabular}[c]{@{}l@{}}100ms \\ / 10Hz\end{tabular}                                            & $\sim$10,000 arcsecs                                                                                     \\
\cellcolor[HTML]{656565}{\color[HTML]{EFEFEF} \begin{tabular}[c]{@{}l@{}}2D Kalman Filter\\  (2D-KF)\end{tabular}}       & 2D                                                                            & \begin{tabular}[c]{@{}l@{}}Only on \\ intialization\end{tabular}                                                   & \begin{tabular}[c]{@{}l@{}}Center of High-Pass \\ Filtered Intensity\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}LCD Screen\\ / Simulation\end{tabular}                                           & \textgreater 5 deg/s                                                                                 & \begin{tabular}[c]{@{}l@{}}1ms \\ / 1kHz\end{tabular}                                              & $\sim$300 arcsecs                                                                                        \\
\cellcolor[HTML]{656565}{\color[HTML]{EFEFEF} \textbf{\begin{tabular}[c]{@{}l@{}}Our Method\\  (EVT-EKF)\end{tabular}}}  & 3D                                                                            & \textbf{\begin{tabular}[c]{@{}l@{}}Only on \\ intialization\end{tabular}}                                          & \textbf{\begin{tabular}[c]{@{}l@{}}Center of Positive Events \\ with Magnitude Offset\end{tabular}}       & \textbf{\begin{tabular}[c]{@{}l@{}}Night Sky with\\ APS Star Tracker\end{tabular}}                          & \textbf{\textgreater 5 deg/s}                                                                        & \textbf{\begin{tabular}[c]{@{}l@{}}1ms \\ / 1kHz\end{tabular}}                                     & \textbf{$\sim$80 arcsecs}                                                                               
\end{tabular}
\end{table*}
